PyTSC: A Unified Platform for Multi-Agent Reinforcement Learning in Traffic Signal Control

Multi-Agent Reinforcement Learning (MARL) presents a promising approach for addressing the complexity of Traffic Signal Control (TSC) in urban environments. However, existing platforms for MARL-based TSC research face challenges such as slow simulation speeds and convoluted, difficult-to-maintain codebases. To address these limitations, we introduce PyTSC, a robust and flexible simulation environment that facilitates the training and evaluation of MARL algorithms for TSC. PyTSC integrates multiple simulators, such as SUMO and CityFlow, and offers a streamlined API, empowering researchers to explore a broad spectrum of MARL approaches efficiently. PyTSC accelerates experimentation and provides new opportunities for advancing intelligent traffic management systems in real-world applications.

==> analysis.tex <==
\section{Analysis}

==> background.tex <==
\section{Background}

\subsection{Decentralized Partially Observable Markov Decision Processes (Dec-POMDPs)}

Decentralized Partially Observable Markov Decision Processes (Dec-POMDPs) represent a foundational framework for modeling multi-agent systems where agents interact with each other and the environment in a decentralized manner, under conditions of partial observability. In the context of traffic signal control (TSC), this formulation becomes highly relevant, enabling a more nuanced analysis of how multiple agents can coordinate their actions to optimize traffic flow. \\
\textbf{Definition} A Dec-POMDP is defined as a tuple 
\(\langle \mathcal{N}, \mathcal{S}, \{\mathcal{A}_i\}, \{\mathcal{O}_i\}, T, \{\Omega_i\}, R \rangle\), where:
\begin{itemize}
    \item \(\mathcal{N}\): A finite set of \(n\) agents, \(\mathcal{N} = \{1, \ldots, n\}\).
    \item \(\mathcal{S}\): A finite set of states that describe the global state of the environment.
    \item \(\{\mathcal{A}_i\}\): A finite set of actions for each agent \(i\), with the joint action space \(\mathcal{A} = \mathcal{A}_1 \times \ldots \times \mathcal{A}_n\).
    \item \(\{\mathcal{O}_i\}\): A finite set of observations for each agent \(i\), with the joint observation space \(\mathcal{O} = \mathcal{O}_1 \times \ldots \times \mathcal{O}_n\).
    \item \(T: \mathcal{S} \times \mathcal{A} \rightarrow \Delta(\mathcal{S})\): A state transition function that maps the current state and joint action to a probability distribution over next states.
    \item \(\{\Omega_i: \mathcal{S} \times \mathcal{A} \rightarrow \Delta(\mathcal{O}_i)\}\): An observation function for each agent, mapping the current state and joint action to a probability distribution over individual observations.
    \item \(R: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}\): A reward function that maps a global state and joint action to a real-valued reward.
\end{itemize}
By capturing the decentralized nature and partial observability inherent in urban traffic systems, Dec-POMDPs offer a foundation for designing intelligent algorithms that can lead to more responsive and efficient traffic signal control. 

\subsection{MARL Frameworks}

The field of Multi-Agent Reinforcement Learning (MARL) has witnessed the development of various frameworks, each designed to tackle the complexities of multi-agent environments. In the realm of Traffic Signal Control (TSC), these frameworks provide unique methodologies to manage decentralized decision-making, partial observability, and agent coordination. Here, we delve into some of the prominent MARL frameworks pertinent to TSC.

\subsubsection{Independent Learning Frameworks}

\paragraph{Independent Q-Learning (IQL)} \cite{tan1993multi} represents a natural extension of the conventional Q-learning algorithm \cite{mnih2015human} to multi-agent settings. In this framework, agents independently learn their respective Q-functions, perceiving other agents as environmental components. Each agent gathers its local history of observations, subsequently updating the Q-value network parameters by minimizing the standard Q-learning loss. Although IQL is conceptually straightforward and easily implementable, it often grapples with non-stationarity issues, as the evolving policies of agents dynamically alter the environment experienced by their counterparts.

\paragraph{Independent synchronous Advantage Actor-Critic (IA2C)} framework is a decentralized training variant of the widely-utilized A2C algorithm \cite{mnih2016asynchronous, baselines}, tailored for multi-agent systems. Within this framework, each agent is equipped with its own actor to approximate the policy, alongside a critic network to estimate the value-function. Both the actor and critic are trained based on the agent's history of local observations, actions, and rewards, with the aim of minimizing the A2C loss. This approach facilitates enhanced coordination among agents, proving beneficial in complex environments such as TSC.

\subsubsection{CTDE Frameworks}

\paragraph{Value Decomposition Networks (VDN)} \cite{sunehag2017value} are designed to linearly decompose the joint Q-value. Agents maintain individual networks to approximate their state-action values, with VDN subsequently decomposing the joint Q-value into the sum of these individual Q-values. The joint state-action values are learned using the standard DQN algorithm \cite{mnih2015human}, with gradients of the joint TD loss backpropagated to each agent's network during training. This methodology retains the advantages of joint action-value functions while maintaining computational efficiency.

\paragraph{QMIX} \cite{rashid2020monotonic} extends VDN to cater to a broader spectrum of environments. It introduces a parameterized mixing network that computes the joint Q-value from the individual state-action value functions of each agent. The mixing network ensures that the global Q-value is a monotonic function of the individual Q-values. QMIX is trained to minimize the DQN loss, with gradients backpropagated to the individual Q-values. This makes QMIX particularly suitable for TSC scenarios, where traffic signals need to synchronize their actions to optimize traffic flow.

\paragraph{Multi-Agent A2C (MAA2C)} is an actor-critic algorithm where the critic learns a joint state value function. It extends the existing on-policy actor-critic algorithm A2C by incorporating centralized critics conditioned on the state of the environment, as opposed to the individual history of observations. MAA2C strikes a balance between cooperative behavior and individual optimization, rendering it a promising framework for TSC.
    
% \item \textbf{Decentralized MARL with Networked Agents}
%     Networked Markov Multi-agent Markov Decision Processes (Networked MMDPs) present a vital and generalized model in the domain of decentralized Multi-Agent Reinforcement Learning (MARL) with networked agents. This framework builds upon the common-reward cooperative model and adds an essential layer of complexity by introducing time-varying communication networks that connect all agents.
%     A networked MMDP is defined by a tuple $<N, S, \{A^{i}\}_{i \in N}, P, \{R^{i}\}_{i \in N}, \gamma, \{G_{t}\}_{t \geq 0}>$, where $N = \{ 1, \cdots, |N| \}$ is the set of $N > 1$ agents, $S$ is the state space observed by all agents, $P: S \times A \rightarrow \Delta(S)$ is the transition probability from any state $s \in S$ to any state $s' \in S$ for any joint action $a \in A$, $A^{i} := A^{1} \times \cdots \times A^{N}$ is the action space for agent $i$, $R^{i}: S \times A \times S \rightarrow \mathbb{R}$ is the reward function that determines the immediate reward received by agent $i$, $\gamma$ is the discount factor, and $G_{t} = <N, E_{t}>$ represents the time-varying communication network. Here, $E_{t}$ is the set of communication links at time $t$, and an edge $(i, j)$ for agents $i, j \in N$ is in $E_{t}$ if agents $i$ and $j$ can communicate with each other at that time.
%     Extending traditional MDPs to multi-agent Markov games, in networked MMDPs, agents aim to cooperatively optimize the long-term return corresponding to the team-average reward:
%     \begin{equation}
%         \bar{R}(s, a, s') := \frac{1}{N} \cdot \sum_{i \in N} R^{i}(s, a, s')
%     \end{equation}
%     for any $(s, a, s') \in S \times A \times S$.
%     This formulation maintains cooperation among agents but allows for different reward functions. The individual agents make decisions utilizing only local information, including data transmitted from neighboring agents over the network. The networked MMDP model not only captures more heterogeneity and privacy among agents but also facilitates the development of decentralized MARL algorithms with only neighbor-to-neighbor communications. Such heterogeneity calls for the incorporation of more efficient communication protocols into MARL, addressing an essential and relatively open problem that naturally arises in networked MMDPs.
%     Through the lens of traffic signal control, networked MMDPs present an opportunity to model the intricate inter-dependencies between different intersections, allowing for more refined and context-aware control strategies. The introduction of networked communication in this model provides an expressive and flexible framework to represent real-world traffic scenarios, opening up new avenues for optimization and coordination in urban traffic management.
    
% \paragraph{\textcolor{red}{[Emergence of MARL in TSC]}} 
%     \begin{itemize}
%         \item In the search for innovative solutions to the challenges of TSC, Multi-Agent Reinforcement Learning (MARL) has emerged as a promising contender. 
%         \item MARL operates on the principle of multiple agents learning and interacting within a shared environment. In the context of TSC, each traffic signal can be viewed as an agent, making decisions based on its observations and the feedback it receives. 
%         % \item Need for decentralized decision making and usage of Dec-POMDP framework -- extends the framework of MDP to multi-agent scenarios with partial observability \cite{oliehoek2016concise}. It is defined by a tuple of $\mathcal{M} = <\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathit{\Omega}, \mathcal{O}, \mathit{r}, \mathcal{N}, \mathit{\gamma}>$, where $\mathit{s} \in \mathcal{S}$ is the global state space and $\mathit{i} \in \mathcal{N} \equiv \{ 1, \cdots, n \}$ is the finite set of agents. At time step $t$, each agent $a$ selects an action $a^{i} \in \mathcal{A}$ resulting in a joint action vector $a \in \mathbf{\mathcal{A}} \equiv \mathcal{A}^{n}$. The transition dynamics of the environment state are given by $\mathit{P}(s'|s, a)$. All agents receive a shared reward according to the reward function $r(s, a)$ and $\gamma \in [0, 1)$ is the discount factor. Each agent receives an observation $o^{a} \in \Omega$ according to the observation function $O(s, a)$. Each agent has an action-observation history $\tau^{i} \in \mathcal{T} \equiv (\mathit{\Omega} \times \mathcal{A})^{*}$ on which it conditions its individual policy $\pi^{i}(a^{i}|\tau^{i})$. The joint policy $\boldsymbol{\pi} = <\pi^{1}, \cdots, \pi^{n}>$ induces a joint-action value function $$Q^{\pi}(s, \mathbf{a}) = E_{s_{0:\infty};\mathbf{a}_{0:\infty}} \left[ \sum_{t=0}^{\infty} \gamma^{t}r_{t}|s_{0} = s; \mathbf{a}_{0} = \mathbf{a}, \boldsymbol{\pi} \right].$$
%         \item \textbf{Decentralized Partially Observable Markov Decision Processes (Dec-POMDPs)}
%             Decentralized Partially Observable Markov Decision Processes (Dec-POMDPs) represent a foundational framework for modeling multi-agent systems where agents interact with each other and the environment in a decentralized manner, under conditions of partial observability. In the context of traffic signal control (TSC), this formulation becomes highly relevant, enabling a more nuanced analysis of how multiple agents can coordinate their actions to optimize traffic flow. \\
%             \textbf{Formal Definition}
%             A Dec-POMDP is defined as a tuple 
%             \(\langle \mathcal{N}, \mathcal{S}, \{\mathcal{A}_i\}, \{\mathcal{O}_i\}, T, \{\Omega_i\}, R \rangle\), where:
%             \begin{itemize}
%                 \item \(\mathcal{N}\): A finite set of \(n\) agents, \(\mathcal{N} = \{1, \ldots, n\}\).
%                 \item \(\mathcal{S}\): A finite set of states that describe the global state of the environment.
%                 \item \(\{\mathcal{A}_i\}\): A finite set of actions for each agent \(i\), with the joint action space \(\mathcal{A} = \mathcal{A}_1 \times \ldots \times \mathcal{A}_n\).
%                 \item \(\{\mathcal{O}_i\}\): A finite set of observations for each agent \(i\), with the joint observation space \(\mathcal{O} = \mathcal{O}_1 \times \ldots \times \mathcal{O}_n\).
%                 \item \(T: \mathcal{S} \times \mathcal{A} \rightarrow \Delta(\mathcal{S})\): A state transition function that maps the current state and joint action to a probability distribution over next states.
%                 \item \(\{\Omega_i: \mathcal{S} \times \mathcal{A} \rightarrow \Delta(\mathcal{O}_i)\}\): An observation function for each agent, mapping the current state and joint action to a probability distribution over individual observations.
%                 \item \(R: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}\): A reward function that maps a global state and joint action to a real-valued reward.
%             \end{itemize}
%             The Dec-POMDP framework introduces several challenges in the context of MARL, such as non-trivial coordination, scalability, and exploration under uncertainty. Agents must learn to cooperate without direct communication and must infer the actions of other agents through indirect observations. This makes the formulation highly expressive but also computationally demanding. In the specific domain of TSC, Dec-POMDPs provide a means to model intricate interactions between traffic signals, vehicles, and road conditions. By capturing the decentralized nature and partial observability inherent in urban traffic systems, Dec-POMDPs offer a foundation for designing intelligent algorithms that can lead to more responsive and efficient traffic signal control. Dec-POMDPs present a rigorous mathematical framework to study the decentralized coordination of agents operating under partial observability. By aligning closely with the real-world complexities of traffic systems, this framework plays a pivotal role in understanding and optimizing traffic signal control using multi-agent reinforcement learning. It catalyzes research directions that embrace both theoretical insights and practical innovations, bridging the gap between abstract models and tangible urban applications.
%         \item \textbf{Decentralized MARL with Networked Agents}
%             Networked Markov Multi-agent Markov Decision Processes (Networked MMDPs) present a vital and generalized model in the domain of decentralized Multi-Agent Reinforcement Learning (MARL) with networked agents. This framework builds upon the common-reward cooperative model and adds an essential layer of complexity by introducing time-varying communication networks that connect all agents.
%             A networked MMDP is defined by a tuple $<N, S, \{A^{i}\}_{i \in N}, P, \{R^{i}\}_{i \in N}, \gamma, \{G_{t}\}_{t \geq 0}>$, where $N = \{ 1, \cdots, |N| \}$ is the set of $N > 1$ agents, $S$ is the state space observed by all agents, $P: S \times A \rightarrow \Delta(S)$ is the transition probability from any state $s \in S$ to any state $s' \in S$ for any joint action $a \in A$, $A^{i} := A^{1} \times \cdots \times A^{N}$ is the action space for agent $i$, $R^{i}: S \times A \times S \rightarrow \mathbb{R}$ is the reward function that determines the immediate reward received by agent $i$, $\gamma$ is the discount factor, and $G_{t} = <N, E_{t}>$ represents the time-varying communication network. Here, $E_{t}$ is the set of communication links at time $t$, and an edge $(i, j)$ for agents $i, j \in N$ is in $E_{t}$ if agents $i$ and $j$ can communicate with each other at that time.
%             Extending traditional MDPs to multi-agent Markov games, in networked MMDPs, agents aim to cooperatively optimize the long-term return corresponding to the team-average reward:
%             \begin{equation}
%                 \bar{R}(s, a, s') := \frac{1}{N} \cdot \sum_{i \in N} R^{i}(s, a, s')
%             \end{equation}
%             for any $(s, a, s') \in S \times A \times S$.
%             This formulation maintains cooperation among agents but allows for different reward functions. The individual agents make decisions utilizing only local information, including data transmitted from neighboring agents over the network. The networked MMDP model not only captures more heterogeneity and privacy among agents but also facilitates the development of decentralized MARL algorithms with only neighbor-to-neighbor communications. Such heterogeneity calls for the incorporation of more efficient communication protocols into MARL, addressing an essential and relatively open problem that naturally arises in networked MMDPs.
%             Through the lens of traffic signal control, networked MMDPs present an opportunity to model the intricate inter-dependencies between different intersections, allowing for more refined and context-aware control strategies. The introduction of networked communication in this model provides an expressive and flexible framework to represent real-world traffic scenarios, opening up new avenues for optimization and coordination in urban traffic management.
%         \item Types of MARL algorithms and their description
%         \begin{itemize}
%             \item Independent Learning: IQL, IA2C
%             \item Centralized Training Decentralized Execution (CTDE): VDN, QMIX, MAA2C
%         \end{itemize}
%         \item The inherent need for traffic signals to coordinate and optimize traffic flow across a network aligns seamlessly with the capabilities of MARL, offering a dynamic and adaptive approach to TSC.
%     \end{itemize}

% \paragraph{Traffic Signal Control as a Multi-agent Markov Game}
% \begin{itemize}
%     \item TSC when viewed through the lens of reinforcement learning, can be formulated as a Markov game where each traffic signal or intersection can be considered as an agent making decisions in the environment. 
%     \item Why is decentralized control necessary for the problem of TSC?
%     \item Decentralization implies partial observability
%     \item Partial observability in TSC implies that each traffic signal uses locally available information to make decisions
%     \item Dec-POMDPs provide a decentralized framework for multi-agent stochastic games with partial observability
%     \item \textbf{Observation space:} The observation for each traffic signal consists of: the number of vehicles $\{ n_{l} \}_{l=1}^{L_{i}}$, the average normalized speed of the vehicles $\{ s_{l} \}_{l=1}^{L_{i}}$, the number of halted vehicles (queue lengths) $\{ q_{l} \}_{l=1}^{L_{i}}$, and the current \texttt{phaseID} of the traffic signal, where $L_{i} \in L$ are the incoming lanes for a traffic signal $i$ and $L$ is a set of all the lanes in the network.
%     \item \textbf{Action space:} For each traffic signal $i$, we define its action $a_{i}$ as choosing one green phase from a list of available phases. As an example, shows the list of phases that are available for a traffic signal in a $4 \times 4$ grid network. A traffic signal can select green phases in (1) any order (implicitly chosen by the agent) or (2) a cyclic or round-robin manner. \footnote{We choose round-robin manner of switching phases for the purpose of benchmarking.} Every green phase must be followed by the corresponding yellow phase, which is enforced by the environment. The duration of yellow phase is fixed to 5 seconds. This scheme is supposed to approximate 3 seconds of yellow time and 2 seconds of red clearance or all red time. Each traffic signal takes an action every 5 simulation seconds.
%     \item \textbf{Reward function:} We chose queue length $q_{l}$ as the performance metric of the traffic signal controller due to its simplistic nature and its property of representing an instantaneous feedback signal. We define the objective function as minimizing the number of vehicles stopped throughout the network where $r_{t} \in \mathbb{R}$ is the global reward and $l \in L$ represents the lanes in the network.
% \end{itemize}

\subsection{Traffic Signal Control as a Multi-agent Markov Game}

\sloppy Traffic Signal Control (TSC) can be conceptualized within the reinforcement learning paradigm as a Markov game. Within this framework, each traffic signal or intersection is perceived as an individual agent, dynamically making decisions based on its interactions with the surrounding environment. A salient feature of this approach is the emphasis on decentralized control. The importance of decentralization in TSC cannot be overstated. By allowing each traffic signal to operate based on locally available information, decisions become acutely responsive to immediate traffic conditions. Furthermore, decentralization is pivotal for ensuring scalability, especially in expansive and intricate urban traffic networks. This decentralized approach inherently introduces an element of partial observability. In essence, while each traffic signal is making decisions, it doesn't possess a holistic view of the entire traffic network. Instead, it relies on localized observations. We define the components of the game as follows:
\begin{itemize}
    \item \textbf{Observation Space:} For each traffic signal, the observation encompasses several critical metrics. Specifically, the observation for each traffic signal consists of: the number of vehicles $\{ n_{l} \}_{l=1}^{L_{i}}$, the average normalized speed of the vehicles $\{ s_{l} \}_{l=1}^{L_{i}}$, the number of halted vehicles (queue lengths) $\{ q_{l} \}_{l=1}^{L_{i}}$, and the current \texttt{phaseID} of the traffic signal. Here, $L_{i} \in L$ represents the incoming lanes for a traffic signal $i$, and $L$ denotes the set of all lanes in the network.
    \item \textbf{Action Space:} The action for each traffic signal $i$ is defined as selecting one green phase from a list of available phases. Traffic signals can either select green phases in any desired order or follow a cyclic or round-robin pattern. \footnote{We choose round-robin manner of switching phases for the purpose of benchmarking.} Notably, every green phase is mandatorily succeeded by its corresponding yellow phase, a constraint enforced by the environment. The yellow phase duration is set at 5 seconds, approximating 3 seconds of yellow and an additional 2 seconds of all-red clearance. Actions are typically taken at intervals of 5 simulation seconds.
    \item \textbf{Reward Function:} The reward function is defined by the queue length metric $q_{l}$, chosen for its inherent simplicity and its capacity to provide instantaneous feedback. The overarching objective, guided by this reward function, is to minimize the number of halted vehicles across the network $r_{t} = \sum_{L}q_{l},$ where $r_{t} \in \mathbb{R}$ represents the global reward and $l \in L$ denotes the lanes in the network.
\end{itemize}




==> related_work.tex <==
\section{Related Work}

% \paragraph{\textcolor{red}{Existing Simulation Environments}}
%     \begin{itemize}
%         \item To facilitate the study and development of advanced TSC strategies, simulation environments play a pivotal role.
%         \item Among the myriad available, SUMO and CityFlow have carved a niche for themselves. 
%         \item These environments offer researchers a realistic representation of traffic dynamics, coupled with the flexibility to integrate various learning algorithms.
%         \item Their popularity can be attributed to their robustness, accuracy, and the ease with which they can be tailored to specific research needs.
%     \end{itemize}

% \paragraph{\textcolor{red}{Benchmarking in TSC}} 
%     \begin{itemize}
%         \item While the tools and techniques for TSC have seen significant advancements, one area that remains under-addressed is benchmarking.
%         \item A comprehensive benchmarking system is crucial for evaluating the efficacy of different MARL approaches, especially as newer algorithms, such as CTDE, come into the fray.
%         \item The current landscape, marked by a dearth of standardized benchmarking tools, poses challenges for researchers.
%         \item It becomes arduous to draw meaningful comparisons, assess the strengths and weaknesses of different approaches, and build upon existing knowledge. 
%         \item This gap underscores the need for a unified benchmarking framework to propel the field forward.
%     \end{itemize}
    
\paragraph{\textcolor{red}{[Existing MARL Frameworks for TSC]}}
The realm of Traffic Signal Control (TSC) has witnessed the emergence of several Multi-Agent Reinforcement Learning (MARL) frameworks, each bringing its unique set of features and capabilities to the table.
\begin{itemize}
    \item Notable among these MARL frameworks are those that have been specifically tailored for TSC applications. These frameworks, while showcasing innovative features, also come with their set of limitations. For instance, while some excel in handling large-scale traffic scenarios, others might be more adept at real-time adaptability.
    \item In terms of benchmarking, a few platforms and datasets have become the go-to choices for many of these frameworks. These benchmarking tools offer a means to evaluate and compare the performance of different MARL strategies in TSC scenarios.
    \item A critical aspect of these frameworks is how they tackle challenges like scalability, ensuring that the system can handle larger, more complex traffic networks. Modularity, allowing for easy integration of new features or algorithms, and real-world applicability, ensuring the solutions are not just theoretically sound but also practically implementable, are also vital considerations.
\end{itemize}
\freefootnote{\url{https://github.com/cts198859/deeprl\_network/}}
\freefootnote{\url{https://github.com/LucasAlegre/sumo-rl}}
\freefootnote{\url{https://github.com/traffic-signal-control/sample-code/}}
\freefootnote{\url{https://github.com/Pi-Star-Lab/RESCO/}}

\paragraph{\textcolor{red}{[Simulation Environments in TSC]}}
Simulation environments serve as the testing grounds for TSC strategies, offering a virtual space where algorithms can be trained, tested, and refined.
\begin{itemize}
    \item Among the plethora of available simulators, SUMO and CityFlow have gained significant traction. Their appeal lies in their ability to closely mimic real-world traffic dynamics, user-friendly interfaces, and the ease with which they can be integrated with MARL algorithms.
    \item However, no tool is without its limitations. While these simulators offer realism, they sometimes fall short in areas like comprehensive benchmarking. The speed of simulation, especially in large-scale TSC scenarios, and the depth of configurability, can also be areas of concern.
    \item Efforts have been made to seamlessly integrate these simulators with MARL frameworks. While some of these integrations have been successful, challenges, primarily stemming from the inherent complexities of both MARL and TSC, persist.
\end{itemize}

\paragraph{\textcolor{red}{[Advancements in CTDE Algorithms]}}
Centralized Training with Decentralized Execution (CTDE) algorithms represent a newer wave of strategies being explored in the TSC domain.
\begin{itemize}
    \item Recent years have seen significant advancements in CTDE algorithms, with researchers exploring their potential in TSC scenarios. These algorithms, by design, are well-suited to address challenges like handling vast state and action spaces and ensuring coordination among multiple agents.
    \item Benchmarking has been a crucial aspect of evaluating the performance of CTDE algorithms in TSC. While some efforts have been made in this direction, comprehensive benchmarking, especially in real-world scenarios, remains an area ripe for exploration.
\end{itemize}

\paragraph{\textcolor{red}{[Benchmarking Methodologies in TSC]}}
Benchmarking is the compass that guides TSC research, offering a means to evaluate, compare, and refine strategies.
\begin{itemize}
    \item Existing benchmarking methodologies vary in their approach. While some focus on specific metrics like throughput or delay, others might take a more holistic approach. Regardless of the approach, the emphasis is always on ensuring that results are reproducible and reflective of real-world performance.
    \item A significant challenge in the TSC community is the lack of standardized benchmarking, especially when it comes to evaluating newer algorithms like CTDE. This absence of standardization can lead to fragmented results, making it challenging to draw broad conclusions or compare different strategies.
    \item Recognizing this gap, there have been recent endeavors to establish more comprehensive and standardized benchmarking platforms for TSC. These efforts aim to provide the community with reliable tools to evaluate and compare the myriad of TSC strategies being developed.
\end{itemize}


